Grasping for a Purpose: Using Task Goals for Efficient Manipulation Planning

In this paper we propose an approach for efficient grasp selection for manipulation tasks of unknown objects. Even for simple tasks such as pick-and-place, a unique solution is rare to occur. Rather, multiple candidate grasps must be considered and (potentially) tested till a successful, kinematically feasible path is found. To make this process efficient, the grasps should be ordered such that those more likely to succeed are tested first. We propose to use grasp manipulability as a metric to prioritize grasps. We present results of simulation experiments which demonstrate the usefulness of our metric. Additionally, we present experiments with our physical robot performing simple manipulation tasks with a small set of different household objects.

==> bimanualOperations.tex <==
In this section we showcase the importance of prioritizing grasps by 
using our approach in a more complex problem: Bimanual pick and place.
In this kind of problem, \Tf{w}{s} and \Tf{w}{g} are located each
within the workspace of a different arm.


%^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^
\begin{figure}[h]
  %\vspace{-1.0em}
\begin{center}
  \begin{tikzbox} {
  \begin{tikzpicture}[minimum width=0]
  	\tikzstyle{label} = [node distance = 1.7cm,text=blue]
    \tikzstyle{mycoord} = [node distance = 0cm]
    \tikzstyle{block} = [node distance = 3.5cm,rounded corners=.00cm,
    inner sep=.1cm, fill=bgcolor, minimum height=2em,minimum width=7em]
    \node[block,name=cover] {\includegraphics[width=0.4\textwidth]{./figures/bimSequence.png} };
  \end{tikzpicture}
  }\end{tikzbox}
\caption{Sample Plan for a Bimanual Pick and Place problem}
\label{fig:bimanualExample}
\end{center}
\vspace{-1.0em}
\end{figure}
%^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^

==> discussion.tex <==
Finally
